Zero-Shot Information Extraction as a Unified Text-to-Triple Translation

We cast a suite of information extraction tasks into a text-to-triple translation framework. Instead of solving each task relying on task-specific datasets and models, we formalize the task as a translation between task-specific input text and output triples. By taking the task-specific input, we enable a task-agnostic translation by leveraging the latent knowledge that a pre-trained language model has about the task. We further demonstrate that a simple pre-training task of predicting which relational information corresponds to which input text is an effective way to produce task-specific outputs. This enables the zero-shot transfer of our framework to downstream tasks. We study the zero-shot performance of this framework on open information extraction (OIE2016, NYT, WEB, PENN), relation classification (FewRel and TACRED), and factual probe (Google-RE and T-REx). The model transfers non-trivially to most tasks and is often competitive with a fully supervised method without the need for any task-specific training. For instance, we significantly outperform the F1 score of the supervised open information extraction without needing to use its training set.

==> tables/cfcorpus.tex <==
\begin{table*}[]
\begin{tabular}{|l|c|}
\hline
Dataset        & Accuracy \\ \hline
OIE2016        &          \\ \hline
WEB            &          \\ \hline
NYT            &          \\ \hline
PENN           &          \\ \hline
CaRB           &          \\ \hline
Wire57         &          \\ \hline
Google-RE-LAMA &          \\ \hline
T-REx-LAMA     & 0.893      \\ \hline
\end{tabular}
\caption{\focus{\small Performance of classification based confidence function trained on T-REx (without T-REx-LAMA). Accuracy is measured with both postive and negative examples.\haoyun{add}}}
\label{tab:newcfcorpus}
\end{table*}

\begin{table*}[]
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{3}{*}{Dataset} & \multicolumn{4}{c|}{Pretrained Corpus}                                                                                            \\ \cline{2-5} 
                         & \multicolumn{2}{c|}{T-REx}                                      & \multicolumn{2}{c|}{OIE2016}                                    \\ \cline{2-5} 
                         & \multicolumn{1}{l|}{Top-1 Acc} & \multicolumn{1}{l|}{Top-5 Acc} & \multicolumn{1}{l|}{Top-1 Acc} & \multicolumn{1}{l|}{Top-5 Acc} \\ \hline
OIE2016                  &  1.0000                        & 1.0000                            &    1.0000                 &   1.0000                             \\ \hline
WEB                      &                                &                                &                                &                                \\ \hline
NYT                      &                                &                                &                                &                                \\ \hline
PENN                     &                                &                                &                                &                                \\ \hline
CaRB                     &                                &                                &                                &                                \\ \hline
Wire57                   &                                &                                &                                &                                \\ \hline
Google-RE-LAMA                &      0.9996                       &                1.0000                &    0.9995                            &        1.0000                        \\ \hline
T-REx-LAMA                    &     0.9917                          &           1.0000                     &   0.9912                             &       0.9996                         \\ \hline
ConceptNet-LAMA               &      1.0000                          &      1.0000                          &    1.0000               &   1.0000                  \\ \hline
\end{tabular}
\caption{\focus{\small Performance of confidence function trained on T-REx (without T-REx-LAMA) and OIE2016 train set.\haoyun{add}}}
\label{tab:cfcorpus}
\end{table*}

==> tables/cfoie.tex <==

\begin{table*}[]
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{2}{*}{System}                 & \multicolumn{4}{c|}{OIE2016} \\ \cline{2-5} 
                                        & P    & R    & F1    & AUC    \\ \hline
Open IE4-confidence                     &      &      &       &        \\ \hline
RnnOIE-confidence                       &      &      &       &        \\ \hline
DeepKnow-BERT$_{\rm{LARGE}}$-confidence &      &      &       &        \\ \hline
\method-BERT$_{\rm{LARGE}}$             &      &      &       &        \\ \hline
\end{tabular}
\caption{\focus{\small Performance of best Open IE systems with confidence functions on the OIE2016 test sets.\zui{add}}}
\label{tab:cfoie}
\end{table*}


